Explicit Birational Geometry of Fano threefold complete intersections

We complete the analysis on the birational rigidity of quasismooth Fano 3-fold deformation families appearing in the Graded Ring Database as a complete intersection. When such a deformation family $X$ has Fano index at least 2 and is minimally embedded in a weighted projective space in codimension 2, we determine which cyclic quotient singularity is a maximal centre. If a cyclic quotient singularity is a maximal centre, we construct a Sarkisov link to a non-isomorphic Mori fibre space or a birational involution. This allows, in particular, the construction of new examples of Fano 3-folds of codimension 6 which are realised as complete intersections in fake weighted projective spaces. We define linear cyclic quotient singularities on $X$ and prove that these are maximal centres by explicitly computing Sarkisov links centred at them. It turns out that each $X$ has a linear cyclic quotient singularity leading to a new birational model. As a consequence, we show that if $X$ is birationally rigid then its Fano index is 1. If the new birational model is a strict Mori fibre space, we determine its fibration type explicitly. In this case, a general member of $X$ is birational to a del Pezzo fibration of degrees 1, 2 or 3 or to a conic bundle $Y/S$ where $S$ is a weighted projective plane with at most $A_2$ singularities.

==> Abstract.tex <==
\section*{Abstract}  \label{sect:abs}

We complete the analysis on the birational rigidity of quasismooth Fano 3-fold deformation families appearing in the Graded Ring Database as a complete intersection. When such a deformation family $X$ has Fano index at least 2 and is minimally embedded in a weighted projective space in codimension 2, we determine which cyclic quotient singularities are maximal centres. If a cyclic quotient singularity is a maximal centre, we construct a Sarkisov link to a non-isomorphic Mori fibre space or a birational involution. We define linear cyclic quotient singularities with respect to $X$ and prove that these are maximal centres by explicitly computing Sarkisov links centred at them. It turns out that each of these deformation families has a linear cyclic quotient singularity leading to a new birational model. As a consequence, we show that if $X$ is birationally rigid then its Fano index is 1. If the new birational model is a strict Mori fibre space, we determine its fibration type explicitly. In this case, a general member of $X$ is birational to a del Pezzo fibration of degrees 1, 2 or 3 or to a conic bundle $Y/S$ where $S$ is a weighted projective plane with at most $A_2$ singularities.  
%complete intersection Fano 3-fold deformation families whose general member is not a cone.

==> MainTheorem.tex <==
\section{Main results}  \label{sect:mainthm}

In this section we present our main results. Let 
\[
X \hookrightarrow \mathbb{P}(a_0,\ldots,a_5)
\]
be a Fano 3-fold deformation family embedded with codimension 2 and Fano index at least two. There are 40 such deformation families which we label by $I=\{86, \ldots,125\}$, see \cite{brownsuI,brownsuII}. We sometimes abuse notation and say $X\in I$ to mean that $X$ is member of a deformation family indexed by $I$. Excluded from the analysis is Family 86: The smooth complete intersection of two quadrics in $\mathbb{P}^5$ which is known to be rational. See for instance \cite{2quadr}.

Let
\begin{align*}
I_{Cb}&=\{87,112,113,118,119\}\\
I_{dP}&=\{88,89,90,91,103,114,116,120,121,122,123,124,125\}
\end{align*}
and
\begin{align*}
I_{nS}&=I_{Cb} \cup I_{dP}\\
I_{S}&=I \setminus I_{nS}.
\end{align*}

The main theorem of this paper is the following:

\begin{Thm} \label{thm:main}
Let $X\subset \mathbb{P}$ be a quasismooth member of a family in $I$. 
\begin{enumerate}
	\item If $X \in I_{nS}$ then $X$ is not solid. In particular,
	\begin{enumerate}
		\item if $X \in I_{Cb}$ then there is a Sarkisov link from $X$ to a conic bundle.
		\item if $X \in I_{dP}$ then there is a Sarkisov link from $X$ to a del Pezzo fibration whose generic fibre has degree 1, 2 or 3.
	\end{enumerate}
		\item If $X \in I_{S}$ then there is a Sarkisov link from $X$  to a terminal non-quasismooth weighted hypersurface or codimension 2 Fano 3-fold.
\end{enumerate}
\end{Thm}

A few words about Theorem \ref{thm:main} and the notation used: We say that $X \in I_{nS}$ if the \emph{general} member 
of that family is in $I_{nS}$. It may happen that only a special member of $X$ is in $I_{nS}$, in which case we rather say $X \in I_S$.
A member in $I_{nS}$ admits a structure of a strict Mori Fibre Space. These are said to be non-solid. See \cite{pfaff}. It is possible for a member in $I_{nS}$ to be birational to weighted hypersurface or codimension 2 Fano 3-fold which indeed happens for a few families. Again, we use the convention that, whenever a general member of $X\in I_{nS}$ admits a structure of a strict Mori Fibre Space, then $X$ is to be indexed in $I_{nS}$. On the other hand, we conjecture that if $X \in I_S$, then $X$ does not a admit such a structure, and is, therefore, solid. Another way to say this is $X \in I_S \implies X \not \in I_{nS}$. Notice, however, that theorem \ref{thm:main} is a statement about quasismooth members of a given family rather than just a statement about the general member.  

The following are immediate consequences of Theorem \ref{thm:main}.
\begin{Cor}
Let $X \in I$. Then $X$ is birationally non-rigid. 
\end{Cor}

\begin{Cor}
There are exactly 19 quasismooth Fano 3-fold weighted complete intersections of codimension 2 which are birationally rigid and they all have index 1. 
\end{Cor}

In fact, theorem \ref{thm:main} can be strengthened to say that if $X \in I_{nS}$ then $X$ is birational to a non-quasismooth weighted hypersurface. Together with \cite{okadaI} this implies in particular that for any quasismooth $X \subset \mathbb{P}(a_0, \ldots, a_5)$ which is not a linear cone, there exists a strict Mori fibration  or a terminal hypersurface which is a birational model of $X$. However, due to time and space constraints we do not present this part of our work here.


%Let $\mathcal{P}(X)$ denote the pliability of $X$.

%\begin{Cor}
%Let $X$ be a quasismooth member of $I_{F}$. Then $|\mathcal{P}(X)| \geq 3$. \textcolor[rgb]{1,0,0}{This is true except for very few cases... detail them} 
%\end{Cor}


Putting together theorem \ref{thm:main} with \cite{chel,okadaI,hamidhyp} and \cite[Example~1.4.4]{3quad} we have a complete picture on the birational rigidity of quasismooth complete intersection Fano 3-folds whose general member is not a cone:
\begin{Thm}
Let $X$ be a quasismooth member of a deformation Fano 3-fold complete intersection whose general member is not a cone. Then $X$ is birationally rigid if and only if $X$ is
\begin{enumerate}
	\item A hypersurface of Fano index 1 or
	\item One of 19 deformation families of Codimension 2 and Fano index 1. 
\end{enumerate}
In particular, if $X$ is birationally rigid it has Fano index 1.
\end{Thm}

Finally, we make the following prediction which will be subject to investigation in the future:

\begin{Conj} \label{conj:solid}
Let $X \in I_S$. Then $X$ is solid.
\end{Conj}

A particular consequence of the above conjecture would be that if $X \in I_S$, then $X$ is not rational.

\subsection*{Organisation of the thesis}

%A further observation coming from this work together with \cite{chel,hamidhyp} for hypersurfaces and \cite{okadaI} for codimension two complete intersections seem to give the general idea that the existence of 

%The following are particular instances of the above conjecture: 

%\begin{Conj}
%\begin{enumerate}%
%	\item Let $X_{6,8} \subset \mathbb{P}$ be a quasismooth member. Then $\mathcal{P}(X_{6,8})= \{X_{6,8}, Z_4, Z_{3,4} \}$ %where $Z_4$ has two coumpound du Val singularities, one being a $cA_2$ singularity, and $Z_{3,4}$ has a $cA_3$ singularity.
%		\item Let $X_{8,10} \subset \mathbb{P}$ be a quasismooth member. Then $\mathcal{P}(X_{8,10})= \{X_{8,10}, Z_5, Z_{4,5} \}$% where $Z_5$ has a $cA_3$ singularity, and $Z_{4,5}$ has some $cDV$ point.
%\end{enumerate}
%\end{Conj}
%\textcolor[rgb]{1,0,0}{
%Obviously need to make the above conjecture precise...
%}

